Tuning Spectral Element Preconditioners for Parallel Scalability on GPUs

The Poisson pressure solve resulting from the spectral element discretization of the incompressible Navier-Stokes equation requires fast, robust, and scalable preconditioning. In the current work, a parallel scaling study of Chebyshev-accelerated Schwarz and Jacobi preconditioning schemes is presented, with special focus on GPU architectures, such as OLCF's Summit. Convergence properties of the Chebyshev-accelerated schemes are compared with alternative methods, such as low-order preconditioners combined with algebraic multigrid. Performance and scalability results are presented for a variety of preconditioner and solver settings. The authors demonstrate that Chebyshev-accelerated-Schwarz methods provide a robust and effective smoothing strategy when using $p$-multigrid as a preconditioner in a Krylov-subspace projector. The variety of cases to be addressed, on a wide range of processor counts, suggests that performance can be enhanced by automated run-time selection of the preconditioner and associated parameters.

==> tables/kershaw-eig-multiplier-0.1.tex <==
\begin{table}
\centering
\begin{tabular}{||c| c c c c c c c c||}
  \hline
  $\lambda_{min}\backslash \lambda_{max}$ & $0.9 \tilde\lambda$ & $0.95 \tilde\lambda$ & $1.0 \tilde\lambda$ & $1.05 \tilde\lambda$ & $1.1 \tilde\lambda$ & $1.15 \tilde\lambda$ & $1.2 \tilde\lambda$ & $1.3 \tilde\lambda$  \\ 
\hline\hline
$0.0 \tilde\lambda$ & 1000 & 1000 & 1000 & 1000 & 1000 & 1000 & 1000 & 1000 \\ 
$0.025 \tilde\lambda$ & 1000 & 1000 & 1000 & 135 & 89 & 81 & 71 & 61 \\ 
$0.05 \tilde\lambda$ & 1000 & 1000 & 121 & 62 & 57 & 53 & 51 & 51 \\ 
$0.1 \tilde\lambda$ & 1000 & 106 & 56 & 54 & 52 & 51 & 52 & 53 \\ 
$0.15 \tilde\lambda$ & 113 & 57 & 55 & 54 & 54 & 54 & 55 & 56 \\ 
$0.2 \tilde\lambda$ & 60 & 58 & 57 & 57 & 57 & 58 & 59 & 60 \\ 
\hline
\end{tabular}
\caption{
  Kershaw ($\varepsilon=0.1, E=26^3, p=7$) iteration counts required to reduce the residual by $10^8$.
  Preconditioner is $p=7,3,1$ p-multigrid V-cycle with a 2nd order Chebyshev-accelerated ASM smoother.
  \label{table:kershaw-eig-multiplier-0.1}}
\end{table}

